Uncertainty Quantification for Neurosymbolic Programs via Compositional Conformal Prediction

Machine learning has become an effective tool for automatically annotating unstructured data (e.g., images) with structured labels (e.g., object detections). As a result, a new programming paradigm called neurosymbolic programming has emerged where users write queries against these predicted annotations. However, due to the intrinsic fallibility of machine learning models, these programs currently lack any notion of correctness. In many domains, users may want some kind of conservative guarantee that the results of their queries contain all possibly relevant instances. Conformal prediction has emerged as a promising strategy for quantifying uncertainty in machine learning by modifying models to predict sets of labels instead of individual labels; it provides a probabilistic guarantee that the prediction set contains the true label with high probability. We propose a novel framework for adapting conformal prediction to neurosymbolic programs; our strategy is to represent prediction sets as abstract values in some abstract domain, and then to use abstract interpretation to propagate prediction sets through the program. Our strategy satisfies three key desiderata: (i) correctness (i.e., the program outputs a prediction set that contains the true output with high probability), (ii) compositionality (i.e., we can quantify uncertainty separately for different modules and then compose them together), and (iii) structured values (i.e., we can provide uncertainty quantification for structured values such as lists). When the full program is available ahead-of-time, we propose an optimization that incorporates conformal prediction at intermediate program points to reduce imprecision in abstract interpretation. We evaluate our approach on programs that take MNIST and MS-COCO images as input, demonstrating that it produces reasonably sized prediction sets while satisfying a coverage guarantee.

==> 10dsl.tex <==

\section{Conformal Queries Over Images}
\label{sec:grammar}

Next, we describe a specific implementation of our approach to construct prediction sets for a query language over images. We describe both the domain-specific language of image queries (Section~\ref{sec:dsl}), as well as the abstract semantics and conformal object predictor that can be used in conjunction with our framework (Section~\ref{sec:abstract-sem}).

\subsection{Domain Specific Language}
\label{sec:dsl}

At a high level, our domain specific language (DSL) takes as input an image, uses an object detector to convert the image into a list of \emph{detections} (which are objects in the image together with their positions), and then uses standard list processing components (e.g., map, filter, and fold) to perform computations over this list. For example, we can express queries such as counting the number of cars in an image, or counting the number of people within 100 pixels of a car.

\paragraph{Type system.}

We first describe the data types associated with our DSL. These data types do not explicitly appear in our DSL, but are the types of components in our DSL; they are also important since we need to construct abstract domains for each of these types. In particular, the type system used by our DSL is the following:
\begin{align*}
\sigma~::=~\textsf{bool}\mid\textsf{int}\mid\textsf{image}\mid\textsf{cat}\mid\sigma\times...\times\sigma\mid\textsf{list}~\sigma\mid\sigma\to\sigma.
\end{align*}
Most of the productions are standard, except $\textsf{image}$ (the type of images, which are 2D integer-valued arrays) and $\textsf{cat}$ (the type of object categories, where object categories are a finite set). We focus on queries involving the categories ``person'' and ``car'', but queries can include additional categories. In addition, we have the derived type
\begin{align*}
\textsf{det}=\textsf{cat}\times\textsf{int}\times\textsf{int}
\end{align*}
representing a detection---i.e., a tuple consisting of an object category together with the $(x,y)$ coordinates of the object in the image. Typically, object detectors output bounding boxes around an image (which is 4D), but our queries only require the center of the bounding box (which is 2D).

\paragraph{Components.}

Our DSL is identical to (\ref{eqn:dsl}), except we use the notation $(f~P~...~P)$ instead of $f(P,...,P)$ since it is more typical for list processing programs:
\begin{align*}
P~::=~X\mid(f~P~...~P)~(f\in\mathcal{F}).
\end{align*}
Next, our DSL includes the follow set $\mathcal{F}$ of components:
\begin{itemize}
\item A machine learning component $\widehat{f}:\textsf{image}\to(\textsf{list}~\textsf{det})$, which is an object detector that takes an image as input and outputs a list of predicted detections in that image. This is the only machine learning component in our DSL (i.e., $\widehat{\mathcal{F}}=\{\widehat{f}\}$).
\item Integers ($0$, $1$, $-1$, $2$, $\cdots$) and Booleans (\textsf{true} and \textsf{false}).
%and list constructors (\textsf{emp} and \textsf{cons}).
\item Arithmetic operators ($+$, $-$, $\times$, $\min$, $\max$, $=$, $\le$, $<$, $\ge$, and $>$), and Boolean operators ($\vee$, $\wedge$, and $\neg$), which have the expected types.
\item List combinators (\textsf{foldr}, \textsf{map}, and \textsf{filter}), which have types
\begin{align*}
\textsf{foldr}&:(\sigma\to\sigma'\to\sigma')\to(\textsf{list}~\sigma)\to\sigma'\to\sigma' \\
\textsf{map}&:(\sigma\to\sigma')\to(\textsf{list}~\sigma)\to(\textsf{list}~\sigma') \\
\textsf{filter}&:(\sigma\to\textsf{bool})\to(\textsf{list}~\sigma)\to(\textsf{list}~\sigma)
\end{align*}
where $\sigma$ and $\sigma'$ are types (technically, list combinators are an infinite set of functions parameterized by $\sigma$ and $\sigma'$).
\end{itemize}
The semantics for these components are standard. Our DSL includes several additional components, such as indexing tuples, taking the product of two lists, functions mapping elements to integers or Boolean constants, etc.; the abstract semantics for these additional constructs are straightforward, so we omit them from our exposition.

\subsection{Abstract Semantics}
\label{sec:abstract-sem}

We now define an abstract semantics $(\mathcal{X}^\#, \alpha, \gamma, \sqcup, \sqcap, \cF^{\#})$ for propagating prediction sets throughout programs. We also describe the conformal object predictor, which outputs abstract lists of detections.

\paragraph{Abstract domains.}

We describe the abstract domain corresponding to each type in our DSL:
\begin{itemize}
\item \textbf{Booleans:} The abstract type $\textsf{bool}^\#$ consists of the constants $\textsf{true}^\#$, $\textsf{false}^\#$, and $\top$ (i.e., either $\textsf{true}$ or $\textsf{false}$).
\item \textbf{Integers:} The abstract type $\textsf{int}^\#=\textsf{int}\times\textsf{int}$ represents closed intervals $[n,m]$ of integers.
\item \textbf{Object categories:} The abstract type $\textsf{cat}^\#=(\textsf{list}~\textsf{cat})$ is a list of categories (the ordering does not matter, so we could also use a set instead of a list).
\item \textbf{Tuples:} The abstract type $(\sigma\times...\times\sigma)^\#=\sigma^\#\times...\times\sigma^\#$ is simply the product of the corresponding abstract base types.
\item \textbf{Lists:} The abstract type $(\textsf{list}~\sigma)^\#=(\textsf{list}~(\sigma^\#\times\textsf{bool}^\#))$ is a list of pairs $(a^\#,b^\#)$ of an abstract value $a^\#$ and a Boolean value $b^\#$. Intuitively, $b^\#$ is a flag indicating whether the element is definitely present in the list ($b^\#=\textsf{true}^\#$), or may or may not be present in the list ($b^\# = \top$).
\item \textbf{Functions:} The abstract type $(\sigma\to\sigma)^\#=\sigma^\#\to\sigma^\#$ is simply a function on abstract values.
\end{itemize}
We do not need an abstract type for images, since they never occur as intermediate program values, only as inputs to machine learning components.
%Within this domain, a prediction interval around an integer is represented by a closed interval on the real line, with two integers as endpoints. A prediction set around a boolean variable is a set of concrete booleans\footnote{Under our syntax, $0 \equiv \{F\}, 1 \equiv \{T\}$, and $? \equiv \{T, F\}$.}. Note the distinction between tuples and lists within our domain is that while  

\paragraph{Conformal object detector.}

%\SP{good to define the scoring fuction here.}

Here, we describe the prediction sets outputted by our conformal object detector.
%we give details on how it is constructed in Section~\ref{sec:conformalobjdet}.
Recall that the object detector $\widehat{f}$ outputs a list of detections---i.e., it has type $\widehat{f}:\textsf{image}\to(\textsf{list}~\textsf{det})$. Thus, the conformal object detector $\widetilde{f}$ outputs an abstract list of detections---i.e., it has type
\begin{align*}
\widetilde{f}:\textsf{image}\to(\textsf{list}~(\textsf{cat}^\#\times\textsf{int}^\#\times\textsf{int}^\#)\times\textsf{bool}^\#).
\end{align*}
In other words, given an image $x$, $\widetilde{f}(x)$ is a list of pairs $(d^\#,b^\#)$, where $b^\#$ indicates whether the object detector is certain that $d^\#$ is an object in $x$. Furthermore, $d^\#=(c^\#,n^\#,m^\#)$ is an abstract detection, where $c^\#$ is a set of object categories, $n^\#$ is an interval around the horizontal position of the center of the object, and $m^\#$ is an interval around its vertical position. Note that in our DSL, images can only occur as the input to an object detector, so we do not need an abstract domain for images.

\paragraph{Abstraction function.}

The abstraction function $\alpha$ converts an element in the concrete domain into a minimal abstract value that contains the concrete value. It is defined as follows:
\begin{itemize}
\item \textbf{Booleans:} We have $\alpha(\textsf{true})=\textsf{true}^\#$ and $\alpha(\textsf{false})=\textsf{false}^\#$.
\item \textbf{Integers:} For an integer $n\in\mathbb{N}$, we have $\alpha(n)=(n,n)$ (which is the abstract value representing the closed interval $[n,n]=\{n\}$).
\item \textbf{Tuples:} Given a tuple $(a_1,...,a_k)$, we have
\begin{align*}
\alpha((a_1,...,a_k))=(\alpha(a_1),...,\alpha(a_k)).
\end{align*}
\item \textbf{Lists:} Given a list $\ell = [a_1, a_2, \cdots, a_k]$, we have
\begin{align*}
\alpha(\ell) = [(\alpha(a_1), \textsf{true}^\#), \cdots, (\alpha(a_k), \textsf{true}^\#)]
\end{align*}
\item \textbf{Functions:} Given a function $f$, we have $\alpha(f)=f^\#$, where $f^\#\in\mathcal{F}^\#$ is the abstract transformer corresponding to $f$. Our DSL only has primitive functions, and does not allow the construction of $\lambda$ terms.
\end{itemize}

\paragraph{Concretization function.}

The concretization function $\gamma$ converts an abstract value into the set of concrete values represented by that abstract value. For our DSL, it is defined as follows:
\begin{itemize}
\item \textbf{Booleans:} We have
\begin{align*}
\gamma(\textsf{true}^\#)&=\{\textsf{true}\} \\
\gamma(\textsf{false}^\#)&=\{\textsf{false}\} \\
\gamma(\top)&=\{\textsf{true},\textsf{false}\}.
\end{align*}
\item \textbf{Integers:} We have $\gamma((\ell,u)) = \{n \in \mathbb{N} \mid \ell \leq n \leq u\}$.
\item \textbf{Tuples:} We have $\gamma((a_1^{\#}, \cdots, a_k^{\#})) = \{(a_1, \cdots, a_k) \mid a_1 \in \gamma(a_1^{\#}), \cdots, a_k \in \gamma(a_k^{\#})\}$.
\item \textbf{Lists:} Given an abstract list $\hat\ell=[(a_1^\#,b_1^\#),...,(a_k^\#,b_k^\#)]$ and a concrete list $\ell=[a_1,...,a_h]$, we have $\ell\in\gamma(\hat\ell)$ iff there exists an injective map $\eta:[h]\to[k]$ (where $[n]=\{1,...,n\}$) such that
\begin{align*}
a_i\in\gamma(a_{\eta(i)}^\#)
\qquad(\forall i\in[h])
\end{align*}
and
\begin{align*}
b_j^\# \neq \textsf{false}^\# \qquad(\forall j\in\text{range}(\eta)) \\
b_j^\# \neq \textsf{true}^\#
\qquad(\forall j\not\in\text{range}(\eta)).
\end{align*}
In other words, there is some sublist of $\hat\ell$ that contains $\ell$, where the Boolean flags for the remaining elements in $\hat\ell$ indicate that they may not be in the list.
\end{itemize}

\paragraph{Join and meet operators.}

The join operator $\sqcup$ takes two abstract values and returns an abstract value that encloses the union of these values. For the application of our framework to the image query DSL, we only ever use $\sqcup$ for abstract values of type $\textsf{int}^{\#}$. Then, for any elements $(\ell_1, u_1), (\ell_2, u_2):\textsf{int}^{\#}$, we have
\begin{align*}
(\ell_1, u_1) \sqcup (\ell_2, u_2) = (\min\{\ell_1, \ell_2\}, \max\{u_1, u_2\}).
\end{align*}
Similarly, the meet operator $\sqcap$ takes two abstract values and returns an abstract value that encodes the intersection of these values. It is given by
\begin{align*}
(\ell_1,u_1) \sqcap (\ell_2,u_2) = (\max\{\ell_1,\ell_2\}, \min\{u_1,u_2\}).
\end{align*}

\paragraph{Abstract transformers.}

The abstract transformers for operators in our DSL are as follows:
\begin{itemize}
\item \textbf{Arithmetic operators:} For $+$, $-$, $\times$, $\min$, $\max$, we have
\begin{align*}
(\ell_1, u_1) +^{\#} (\ell_2, u_2) &= (\ell_1 + \ell_2, u_1 + u_2) \\
(\ell_1, u_1) -^{\#} (\ell_2, u_2) &= (\ell_1 - u_2, u_2 - \ell_1) \\
(\ell_1, u_1) \times^{\#} (\ell_2, u_2) &=
\begin{cases}
(\ell_1 \times \ell_2, u_1 \times u_2) & \text{if } ~ u_1 \geq 0 \text{ and } u_2 \geq 0 \\
(u_1 \times u_2, \ell_1 \times \ell_2) & \text{if } ~ u_1 < 0 \text{ and } u_2 < 0 \\
(\ell_1 \times u_2, \ell_2 \times u_1) & \text{if } ~ u_1 < 0 \text{ and } \ell_2 \geq 0 \\
(u_1 \times \ell_2, u_2 \times \ell_1) & \text{if } ~ \ell_1 \geq 0 \text{ and } u_2 < 0
\end{cases} \\
\textsf{min}^{\#}~((\ell_1, u_1), (\ell_2, u_2)) &= (\textsf{min}~(\ell_1, \ell_2),\textsf{min}~(u_1, u_2)) \\
\textsf{max}^{\#}~((\ell_1, u_1), (\ell_2, u_2)) &= (\textsf{max}~(\ell_1, \ell_2),\textsf{max}~(u_1, u_2)) \\
\end{align*}
For $\ge^{\#}$, $>^{\#}$, and $=^{\#}$ (we omit $\le^\#$ and $<^\#$ since they are similar), we have
\begin{align*}
(\ell_1, u_1) \ge^{\#} (\ell_2, u_2) &= 
\begin{cases}
\textsf{true}^\# & \text{if } \ell_1 \geq u_2 \\
\textsf{false}^\# & \text{if } \ell_2 < u_1 \\
\top & \text{otherwise.}
\end{cases} \\
(\ell_1, u_1) >^{\#} (\ell_2, u_2) &=
\begin{cases} 
\textsf{true}^\# & \text{if } \ell_1 > u_2 \\
\textsf{false}^\# & \text{if } \ell_2 \le u_1 \\
\top & \text{otherwise.}
\end{cases} \\
(\ell_1, u_1) =^{\#} (\ell_2, u_2) &=
\begin{cases}
\textsf{true}^\# & \text{if } \ell_1 = u_1 = \ell_2 = u_2 \\
\textsf{false}^\# & \text{if } u_1 < \ell_2 \vee \ell_1 > u_2 \\
\top & \text{otherwise.}
\end{cases}
\end{align*}
\item \textbf{Boolean operators:} For $\vee^{\#}$, $\wedge^{\#}$, and $\neg^{\#}$. If all inputs are $\textsf{true}^\#$ or $\textsf{false}^\#$, then the semantics are equivalent to those for $\vee$, $\wedge$, and $\neg$, respectively. Otherwise, we have
\begin{align*}
(\top \vee^{\#} \textsf{true}^\#) = (\textsf{true}^\# \vee^{\#} \top) &= \textsf{true}^\# \\
(\top \vee^{\#} \textsf{false}^\#) = (\textsf{false}^\# \vee^{\#} \top) &= \top \\
(\top \wedge^{\#} \textsf{true}^\#) = (\textsf{true}^\# \wedge^{\#} \top) &= \top \\ 
(\top \wedge^{\#} \textsf{false}^\#) = (\textsf{false}^\# ~\wedge^{\#} \top) &= \textsf{false}^\# \\
(\top \wedge^{\#} \top) = (\top \vee^{\#} \top) &= \top \\
\neg^{\#} \top &= \top.
\end{align*}
\item \textbf{List combinators:} First, the abstract transformer for $\textsf{map}$ has type
\begin{align*}
\textsf{map}^\# :  (\sigma \to \sigma')^\# \to (\textsf{list}~\sigma)^\# \to (\textsf{list}~\sigma')^\#,
\end{align*}
and has semantics
\begin{align*}
(\textsf{map}^{\#} ~  f^{\#} ~ [(a_1^{\#}, b_1^\#), \cdots, (a_k^{\#}, b_k^\#)]) = [(f^{\#}(a_1^{\#}), b_1^\#), \cdots, (f^{\#}(a_k^{\#}), b_k^\#)].
\end{align*} \\
Next, the abstract transformer for $\textsf{filter}$ has type
\begin{align*}
\textsf{filter}^\# : (\sigma \to \textsf{bool})^{\#} \to (\textsf{list}~\sigma)^\# \to (\textsf{list}~\sigma)^\#,
\end{align*}
and has semantics
\begin{align*}
(\textsf{filter}^{\#} ~  f^{\#} ~ [(a_1^{\#}, b_1^\#), \cdots, (a_k^{\#}, b_k^\#)]) = [(a_i^{\#}, b_i^\# \wedge^\# f^\#(a_i^\#) \mid f^{\#}(a_i^{\#})\neq\textsf{false}^\#]_{i = 1}^k.
\end{align*}
In other words, it filters out elements such that $f^\#(a_i^\#)=\textsf{false}^\#$; for the remaining elements, the output is definitely in the list iff $a_i^\#$ is definitely in the list (i.e., $b_i^\#=\textsf{true}$) and $f^\#(a_i^\#)$ is definitely equal to \textsf{true} (i.e., $f^\#(a_i^\#)=\textsf{true}^\#$). Finally, the abstract transformer for $\textsf{foldr}$ has type
\begin{align*}
\textsf{foldr}^\# : (\sigma \to \sigma' \to \sigma')^\# \to (\textsf{list}~\sigma)^\# \to \sigma'^\# \to (\textsf{list}~\sigma')^\#,
\end{align*}
and has recursive semantics
\begin{align*}
(\textsf{foldr}^{\#} ~ f^{\#} ~ [(a_1^\#,b_1^\#),\cdots,(a_k^\#,b_k^\#)] ~ c^{\#}) = 
\begin{cases}
c^{\#}  & \text{if } k = 0 \\
\widetilde{c}^\# & \text{if } b_1^\# = \textsf{false}^\# \\ 
f^{\#}(a_1^{\#}, \widetilde{c}^\#) & \text{if } b_1^\# = \textsf{true}^\# \\
\widetilde{c}^\# \sqcup f^{\#}(a_1^{\#}, \widetilde{c}^\#) & \text{if } b_1^\# = \top,
\end{cases}
\end{align*}
where
\begin{align*}
\widetilde{c}^\# = (\textsf{foldr}^{\#} ~ f^{\#} ~ [(a_2^\#,b_2^\#),\cdots,(a_k^\#,b_k^\#)] ~ c^{\#}).
\end{align*}
In other words, if $k=0$ (i.e., the input list is empty) or $b_1^\#=\textsf{true}^\#$, the semantics are equivalent to the standard semantics for $\textsf{foldr}$, but if $b_1^\#= \textsf{false}^\#$, then we ignore $a_1^\#$, and if $b_1^\#= \top $, then it takes the join of the case where $a_1^\#$ is in the list and the case where it is not in the list.
\end{itemize}

% \subsection{Developing a prediction set abstraction}
% \label{subsec:pred-interval-grammar}
% Our goal is to define a general procedure through which we can take any grammar and generate a corresponding abstract syntax and semantics that take prediction sets (rather than point values) as input, and propagate these prediction sets through programs. If a prediction set has a theoretical guarantee of coverage over a true point value at input, we would like it to maintain this guarantee as it propagates through the program and gets modified. \\ \\
% Consider a language defined by grammar $G=(\Sigma,V,S,P)$, and let $L$ be the concrete set values that can be taken by variables in the language. Then, we define the abstract set $L' \subseteq \cP(L)$, as the domain of all definable prediction sets. Assume there exists an abstraction function $\alpha: L \to L'$, which maps every element $x \in L$ to a corresponding abstract value $x' \in L'$, and a concretization function $\gamma: L' \to \cP(L)$, which maps any abstract value $x' \in L'$ to the set of concrete values that $x'$ could represent in the concrete set $L$\footnote{If we were only concerned with mapping "concrete" integers to "abstract" sets of integers, for example, the way $\alpha$ and $\gamma$ work are clear. For instance, $\alpha(2) = \{2\}$, $\gamma(\{2\}) = \{2\}$, and $\gamma(\{2, 3, 4\}) = \{2, 3, 4\}$.}. \\ \\

% \subsection{Abstract Domain}
% \label{subsec:abs-dom}
% The abstract domain consists of elements of type $\widehat{\tau}$, where:
% \begin{align*}
% \widehat{\tau}&::=\widehat{\textsf{bool}}\mid\widehat{\textsf{int}}\mid{\textsf{list}}~\widehat{\sigma} \\
% \widehat{\sigma}&::=\textsf{pair}(\widehat{\tau},\widehat{\textsf{bool}}) \\
% \widehat{\textsf{bool}}&::=0 \mid 1 \mid ~ ? \\
% \widehat{\textsf{int}}&::=\textsf{pair}(\textsf{int},\textsf{int}) 
% \end{align*}
% Notice that any list consists of elements $(c,b)$ of type $\widehat{\sigma}$. The second element $b$ of any member of a list (which will always be either $0$, $1$ or $\{0,1\}$) is a boolean flag. If $b = 1$, this represents our certainty that $c$ is truly a concrete element of the list. If $b = 0$, then $c$ is not an element of the list, and if $b = ~?$, then $c$ could either be or not be a concrete element of the list. The abstract value of an integer represents a range: for any value $(l,u)$ with type $\widehat{\textsf{int}}$, the concrete value of this integer will be in the interval $[l,u]$. \\ \\
% \osbert{Use $\mathcal{L}(C)$ to denote lists of elements in $C$.}
% \paragraph{Abstraction Function.} The abstraction function $\alpha$ \ramya{(How do I define a domain for all possible values of type $\widehat{\tau}$?)} is defined as follows: \\
% For all $b$ of type $\textsf{bool}$,
% \begin{equation*}
%     \alpha(b) = b
% \end{equation*}
% For all $n$ of type $\textsf{int}$,
% \begin{equation*}
%     \alpha(n) = (n,n)
% \end{equation*}
% For all lists $\ell = [a_1, a_2, \cdots, a_n]$,
% \begin{equation*}
%     \alpha(\ell) = [(a_1, 1), (a_2, 1), \cdots, (a_n, 1)]
% \end{equation*}

% \paragraph{Concretization Function.} The concretization function $\gamma$ is defined as follows: \\ \\
% For all $b$ of type $\widehat{\textsf{bool}}$,
% \begin{equation*}
%     \alpha(b) = b
% \end{equation*}
% For all $(l,u)$ of type $\widehat{\textsf{int}}$,
% \begin{equation*}
%     \gamma((l,u)) = \{n \in \mathbb{N} \mid l \leq n \leq u\}
% \end{equation*}
% For all lists $\widehat{\ell} = [(a_1, b_1), (a_2, b_2), \cdots (a_n, b_n)]$, 
% \begin{equation*}
%     \gamma(\widehat{\ell}) = O(\{a_i \in \widehat{l} \mid b_i = 1\} \cup \mathcal{P}(\{a_i \in \widehat{l} \mid b_i \neq 1\})
% \end{equation*}
% where $O$ is an ordering function that, given a subset of $\{a_1, a_2, \cdots a_n\}$ returns an ordered list in ascending order of their indices (required to maintain the ordering of the original list $\ell$). 

% \paragraph{Join Function.} The $\textsf{join}$ function $\sqcup$ takes two abstract values and returns the smallest abstract value that encloses both inputs. For the purposes of this grammar, we will assume that $\textsf{join}$ will only ever take $\widehat{\textsf{int}}$ values as input. For any elements $(l_1, u_1), (l_2, u_2)$ of type $\widehat{\textsf{int}}$,
% \begin{equation*}
%     (l_1, u_1) ~ \sqcup ~ (l_2, u_2) = (\min(l_1, l_2), \max(u_1, u_2))
% \end{equation*}



==> 7_1mnist.tex <==

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{MNIST-resized/example1.png}
\vspace{-1.5\baselineskip}
\caption{sum of list elements}
\label{fig:MNIST-prog-1}
\end{subfigure}
\qquad
%\hfill
\begin{subfigure}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{MNIST-resized/example2.png}
\vspace{-1.5\baselineskip}
\caption{sum of list elements less than 7 }
\label{fig:MNIST-prog-2}
\end{subfigure}
%\vfill \vfill \vfill
\begin{subfigure}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{MNIST-resized/example3.png}
\vspace{-1.5\baselineskip}
\caption{max of list elements}
\label{fig:MNIST-prog-3}
\end{subfigure}
%\hfill
\qquad
\begin{subfigure}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{MNIST-resized/example4.png}
\vspace{-1.5\baselineskip}
\caption{\# of list elements less than 6}
\label{fig:MNIST-prog-4}
\end{subfigure}
%\vfill \vfill \vfill
\begin{subfigure}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{MNIST-resized/example6.png}
\vspace{-1.5\baselineskip}
\caption{\# of list elements equal to 2}
\label{fig:MNIST-prog-5}
\end{subfigure}
%\hfill
\qquad
\begin{subfigure}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{MNIST-resized/example8.png}
\vspace{-1.5\baselineskip}
\caption{\# of list elements between 3 and 8}
\label{fig:MNIST-prog-6}
\end{subfigure}
%\vfill \vfill \vfill
\begin{subfigure}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{MNIST-resized/example5.png}
\vspace{-1.5\baselineskip}
\caption{max sum of any two list elements}
\label{fig:MNIST-prog-7}
\end{subfigure}
\qquad
%\hfill
\begin{subfigure}[b]{0.35\textwidth}
\centering
\includegraphics[width=\textwidth]{MNIST-resized/example7.png}
\vspace{-1.5\baselineskip}
\caption{max distance between any two list elements}
\label{fig:MNIST-prog-8}
\end{subfigure}
\caption{Results for prediction set size across all test-data for all programs in Section \ref{sec:mnist}, ordered in increasing order of size of the composed prediction set result.}
\label{fig:MNIST}
\end{figure}


==> 7_2objdetimgs.tex <==

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example1_ordered.png}
\caption{Program 1}
\label{fig:prog-1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example2_left_ordered.png}
\caption{Program 2}
\label{fig:prog-2}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example2_right_ordered.png}
\caption{Program 3}
\label{fig:prog-3}
\end{subfigure}
\vfill \vfill \vfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example2_top_ordered.png}
\caption{Program 4}
\label{fig:prog-4}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example2_bottom_ordered.png}
\caption{Program 5}
\label{fig:prog-5}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example3_ordered.png}
\caption{Program 6}
\label{fig:prog-6}
\end{subfigure}
\vfill \vfill \vfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example4_ordered.png}
\caption{Program 7}
\label{fig:prog-7}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example5_ordered.png}
\caption{Program 8}
\label{fig:prog-8}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example6_ordered.png}
\caption{Program9}
\label{fig:prog-9}
\end{subfigure}
\vfill \vfill \vfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example7_ordered.png}
\caption{Program 10}
\label{fig:prog-10}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example8_ordered.png}
\caption{Program 11}
\label{fig:prog-11}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{ObjDetection/example9_ordered.png}
\caption{Program 12}
\label{fig:prog-12}
\end{subfigure}
\caption{Results for prediction set size across all test-data for all programs in Section \ref{sec:obj-detect}, ordered in increasing order of size of the composed prediction set result.}
\label{fig:obj-det-imgs}
\end{figure}


==> conformaldet.tex <==

\subsection{Conformal Object Detector}
\label{sec:conformalobjdet}

TODO

\SP{change notations consistently later.}
\begin{itemize}
\item each predicted detection: $\hat{d} = ({\color{red}\hat{s}}, \hat{n}, \hat{m}, {\color{red}\hat{w}, \hat{h}})$\SP{$s, w, h$ are not used so far. $s$ is a distribution over categories}
\item each true detection: $d = (c, n, m)$
%\item detections: we call a detection a predected detection if its category score $s_c$ is larger than or equal to 0.5.
\item matching: for each true detection, choose a detection that maximizes $\text{RoI}$. Note that there is always one match.
\item we denote the list of true detections by $D = (d^{(1)}, \dots, d^{(J)})$ and the list of the matched predicted detections by $\hat{D} = (\hat{d}^{(1)}, \dots, \hat{d}^{(J)})$.

% \item a scoring function for a single detection for $d$:
%  \begin{align*}
%  g(x, d) = \hat{s}_{c} \left( \frac{|n - \hat{n}|}{\hat{w}} + \frac{|m - \hat{m}|}{\hat{h}} \right)
%  \end{align*}
%  \item a scoring function for multiple detections for $d^{(1)}, \dots d^{(J)}$
%  \begin{align*}
%  g(x, (d^{(1)}, \dots, d^{(J)})) = \frac{1}{J} \sum_{j=1}^J \hat{s}_{c^{(j)}}^{(j)} \left( \frac{|n^{(j)} - \hat{n}^{(j)}|}{\hat{w}^{(j)}} + \frac{|m^{(j)} - \hat{m}^{(j)}|}{\hat{h}^{(j)}} \right)
%  \end{align*}
 \item a score function for a ``certain'' category score:
 \begin{align*}
 g_{d_1}(x, (c^{(1)}, \dots, c^{(J)})) = \max_{j} \hat{s}_{c^{(j)}}^{(j)} 
 \end{align*}
 \item a score function for an idk category score:
 \begin{align*}
 g_{d_1'}(x, (c^{(1)}, \dots, c^{(J)})) = \min_{j} \hat{s}_{c^{(j)}}^{(j)} 
 \end{align*}
 \item a score function for a score of x location:
 \begin{align*}
 g_{d_2}(x, (n^{(1)}, \dots, n^{(J)})) = \max_{j}  \frac{|n^{(j)} - \hat{n}^{(j)}|}{\hat{w}^{(j)}} 
 \end{align*}
 \item a score function for a score of y location:
 \begin{align*}
 g_{d_3}(x, (m^{(1)}, \dots, m^{(J)})) = \max_{j} \frac{|m^{(j)} - \hat{m}^{(j)}|}{\hat{h}^{(j)}} 
 \end{align*}
 \item we consider three conformal predictors for each score function along with a composed one:
 \begin{align*}
 \tilde{f}_{d_1}(x) &= \{ C \mid g_{d_1}(x, C) \ge \tau_{d_1} \}
 \\
 \tilde{f}_{d_1'}(x) &= \{ C \mid g_{d_1}(x, C) \ge \tau_{d_1'} \}
 \\
 \tilde{f}_{d_2}(x) &= \{ N \mid g_{d_2}(x, N) \ge \tau_{d_2} \}
 \\
 \tilde{f}_{d_3}(x) &= \{ M \mid g_{d_3}(x, M) \ge \tau_{d_3} \}
 \\
 \tilde{f}(x) &= \{ (C, N, M, B) \mid C \in \tilde{f}_{d_1}(x), C' \in \tilde{f}_{d_1'}(x), N \in \tilde{f}_{d_2}(x), M \in \tilde{f}_{d_3}(x) \}
 \end{align*}
 \item a desired coverage guarantee via a union bound:
 If 
 $\mathbb{P}[ C \in \tilde{f}_{d_1}(x) ] \ge 1 - \delta_{d_1}$, 
 $\mathbb{P}[ C \in \tilde{f}_{d_1}(x) ] \ge 1 - \delta_{d_1'}$, 
 $\mathbb{P}[ N \in \tilde{f}_{d_2}(x) ] \ge 1 - \delta_{d_2}$, 
 $\mathbb{P}[ M \in \tilde{f}_{d_3}(x) ] \ge 1 - \delta_{d_3}$, 
 and
 $\delta = \delta_{d_1} + \delta_{d_1'} + \delta_{d_2} + \delta_{d_3}$,
 then we have
 \begin{align*}
 \mathbb{P} \left[ D \in \tilde{f}(x) \right] \ge 1 - \delta.
 \end{align*}
 \end{itemize}


==> oldstuff.tex <==

\clearpage

Let $\mathcal{T}=\Sigma^\#\times(\Sigma\cup\{\bot\})^n$, and suppose we have a semantics $\den{p}^C_{\epsilon}:\mathcal{T}\to\mathcal{T}$, then its pushforward is a mapping $\den{p}_{\epsilon,*}^C:\mathcal{M}\mathcal{T}\to\mathcal{M}\mathcal{T}$. The denotational semantics are

Assign: $\den{\vec{x}\coloneqq f(\vec{x})}_{\epsilon}^C(\sigma^\#,\sigma_1,...,\sigma_n)=(f^\#(\sigma^\#),f^*(\sigma_1),...,f^*(\sigma_n))$

Assign-hat: $\den{\vec{x}\coloneqq\widehat{f}(\vec{x})}_{\epsilon}^C(\sigma^\#,\sigma_1,...,\sigma_n)=(C_{\epsilon}(\{f^*(\sigma_i)\}_{i=1}^n),f^*(\sigma_1),...,f^*(\sigma_n))$

Sequence: $\den{p;q}_{\epsilon}^C=\den{p}_{\epsilon/2}^C\circ\den{q}_{\epsilon/2}^C$

Conditional: $\den{\textbf{if }x\textbf{ then }p\textbf{ else }q\textbf{ end}}_{\epsilon}^\#(\sigma^\#,\sigma_1,...,\sigma_n)=({\sigma^\#}',...)$

\clearpage

Let $\Sigma=\mathbb{R}^n$ be the space of stores, and $\Sigma^\#$ be the space of abstract stores. Given $f\in\mathcal{F}$, consider the associated standard semantics $f:\Sigma\to\Sigma$, abstract semantics $f^\#:\Sigma^\#\to\Sigma^\#$, and conformal semantics $\widetilde{f}_{\mu,\epsilon}\in\Sigma^\#$. We assume that $f^\#$ satisfies
\begin{align*}
\sigma\in\gamma(\sigma^\#)\Rightarrow f(\sigma)\in\gamma(f^\#(\sigma^\#)),
\end{align*}
and $\widetilde{f}_{\mu,\epsilon}$ satisfies
\begin{align*}
\mathbb{P}_{\mu}[f(\sigma)\in\widetilde{f}_{\mu,\epsilon}]\ge1-\epsilon.
\end{align*}
Now, consider the Markov kernel $F:\Sigma^\#\to\mathcal{M}\Sigma^\#$ defined by
\begin{align*}
F(\sigma^\#)=\delta_{f^\#(\sigma^\#)\sqcap\widetilde{f}_{\mu,\epsilon}},
\end{align*}
and consider its pushforward measure $F_*:\mathcal{M}\Sigma^\#\to\mathcal{M}\Sigma^\#$ defined by
\begin{align*}
F_*(\mu^\#)(B)=\mu^\#(F^{-1}(B))=\mu^\#(\{\sigma^\#\in\Sigma^\#\mid F(\sigma^\#)\in B\}).
\end{align*}
Now, we have
\begin{align*}
\den{\vec{x}\coloneqq f(\vec{x})}^\#_{\epsilon}(\mu^\#)&=F_*(\mu^\#)
\end{align*}
We want to prove that
\begin{align*}
\mathbb{P}_{\mu}\left[\den{p}^*(\sigma)\in\gamma\left(\den{p}_{\epsilon}^\#(\delta_{\alpha(\sigma)})\right)\right]\ge1-\epsilon
\end{align*}

\clearpage
\[\frac{}{\langle\textbf{skip},\sigma,\delta\rangle\Downarrow^\#\langle\sigma,\delta\rangle}~(\text{skip})\] \\
\[\frac{a=f^\#(\sigma(x_1),...,\sigma(x_k))}
{\langle x\gets f(x_1,...,x_k),\sigma,\delta\rangle\Downarrow^\#\langle\sigma[x\mapsto a],\delta\rangle}~(\text{assign})\] \\
\[\frac{a=\tilde{f}_{\delta'}(x_{\text{in}})}
{\langle x\gets\hat{f}(x_1,...,x_k),\sigma,\delta\rangle\Downarrow^\#\langle\sigma[x\mapsto a],\delta+\delta'\rangle}~(\text{assign-hat})\] \\
\[\frac{\langle p,\sigma,\delta\rangle\Downarrow^\#\langle \sigma',\delta'\rangle
\quad\langle p',\sigma',\delta'\rangle\Downarrow^\#\langle\sigma'',\delta''\rangle}
{\langle p;p',\sigma,\delta\rangle\Downarrow^\#\langle\sigma'',\delta''\rangle}~(\text{sequence})\] \\
\[\frac{\sigma(x)=\text{false}}
{\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma,\delta\rangle\Downarrow^\#\langle\sigma,\delta\rangle}~(\text{while-false})\] \\
\[\frac{\sigma(x)=\text{true}
\quad\langle p,\sigma,\delta\rangle\Downarrow^\#\langle\sigma',\delta'\rangle
\quad\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma',\delta'\rangle\Downarrow^\#\langle\sigma'',\delta''\rangle}
{\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma,\delta\rangle\Downarrow^\#\langle\sigma'',\delta''\rangle}~(\text{while-true})\] \\
\[\frac{\sigma(x)=\top
\quad\langle p,\sigma,\delta\rangle\Downarrow^\#\langle\sigma',\delta'\rangle
\quad\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma',\delta'\rangle\Downarrow^\#\langle\sigma'',\delta''\rangle}
{\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma,\delta\rangle\Downarrow^\#\langle\sigma\sqcup\sigma'',\delta''\rangle}~(\text{while-top})\]

\clearpage

\begin{align*}
P~::=~\textbf{skip}
\mid X\gets f(X,...,X)~(f\in\mathcal{F})
\mid P;P
\mid\textbf{while }X\textbf{ do }P\textbf{ end}
\qquad
X~::=~x~(\forall x\in\mathcal{X})
\end{align*}
We assume that $\mathcal{X}$ contains a distinguished, immutable \emph{input variable} $x_{\text{in}}\in\mathcal{X}$.
\[\frac{}{\langle\textbf{skip},\sigma,\sigma_*,F\rangle\Downarrow^\#\langle\sigma,\sigma_*,F\rangle}~(\text{skip})\] \\
\[\frac{a=f^\#(\sigma(x_1),...,\sigma(x_k))
\quad c=f(\sigma_*(x_1),...,\sigma_*(x_k))}
{\langle x\gets f(x_1,...,x_k),\sigma,\sigma_*,F\rangle\Downarrow^\#\langle\sigma[x\mapsto a],\sigma_*[x\mapsto c],F\rangle}~(\text{assign})\] \\
\[\frac{a=f^\#(\sigma(x_1),...,\sigma(x_k))
\quad a'=\tilde{f}_{F,\delta}(x_{\text{in}})
\quad c=f(\sigma_*(x_1),...,\sigma_*(x_k))
\quad E=\mathbbm{1}(c\in\gamma(a'))}
{\langle x\gets f(x_1,...,x_k),\sigma,\sigma_*,F\rangle\Downarrow^\#\langle\sigma[x\mapsto a\sqcap a'],\sigma_*[x\mapsto c],F\circ[(E,\delta)]\rangle}~(\text{assign}')\] \\
\[\frac{a=\tilde{f}_{F,\delta}(x_{\text{in}})
\quad c=f^*(\sigma_*(x_1),...,\sigma_*(x_k))
\quad E=\mathbbm{1}(c\in\gamma(a))}
{\langle x\gets\hat{f}(x_1,...,x_k),\sigma,\sigma_*,F\rangle\Downarrow^\#\langle\sigma[x\mapsto a],\sigma_*[x\mapsto c],F\circ[(E,\delta)]\rangle}~(\text{assign-hat})\] \\
\[\frac{\langle p,\sigma,\sigma_*,F\rangle\Downarrow^\#\langle \sigma',\sigma_*',F'\rangle
\quad\langle p',\sigma',\sigma_*',F'\rangle\Downarrow^\#\langle\sigma'',\sigma_*'',F''\rangle}
{\langle p;p',\sigma,\sigma_*,F\rangle\Downarrow^\#\langle\sigma'',\sigma_*'',F''\rangle}~(\text{sequence})\] \\
\[\frac{\sigma(x)=\text{false}}
{\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma,\sigma^*,F\rangle\Downarrow^\#\langle\sigma,\sigma^*,F\rangle}~(\text{while-false})\] \\
\[\frac{\sigma(x)=\text{true}
\quad\langle p,\sigma,\sigma_*,F\rangle\Downarrow^\#\langle\sigma',\sigma_*',F'\rangle
\quad\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma',\sigma_*',F'\rangle\Downarrow^\#\langle\sigma'',\sigma_*'',F''\rangle}
{\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma,\sigma_*,F\rangle\Downarrow^\#\langle\sigma'',\sigma_*'',F''\rangle}~(\text{while-true})\] \\
\[\frac{\sigma(x)=\top
\quad\langle p,\sigma,\sigma_*,F\rangle\Downarrow^\#\langle\sigma',\sigma_*',F'\rangle
\quad\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma',\sigma_*',F'\rangle\Downarrow^\#\langle\sigma'',\sigma_*'',F''\rangle}
{\langle\textbf{while }x\textbf{ do }p\textbf{ end},\sigma,F\rangle\Downarrow^\#\langle\sigma\sqcup\sigma'',\text{ite}(\sigma_*(x),\sigma_*'',\sigma_*),F''\rangle}~(\text{while-top})\]
Here, $\sigma:\mathcal{X}\to\mathcal{C}^\#$ is a store mapping variables to their (abstract) values, $\delta\in\mathbb{R}_{>0}$ is a positive real number encoding a confidence level, and $F\in\mathcal{F}\coloneqq(\mathcal{E}\times\mathbb{R}_{>0})^*$ is a list of pairs of machine learning models and confidence levels.

Note that the rules only append elements to $F$. Thus, the semantics always have the form $\langle p,\sigma,\sigma^*,F\rangle\Downarrow^\#\langle\sigma',\sigma_*',F\circ F'\rangle$. We prove that for a rule in this form, letting $F=[(E_1,\delta_1),...,(E_n,\delta_n)]$ and $F'=[(E_1',\delta_1'),...,(E_{n'}',\delta_{n'}')]$, then assuming
\begin{align*}
\mathbb{P}[E_i\mid E_1,...,E_{i-1}]\ge1-\delta_i
\qquad(\forall i\in[n]),
\end{align*}
we have
\begin{align*}
\mathbb{P}[E_i'\mid E_1,...,E_n,E_1',...,E_{i-1}']\ge1-\delta_i'
\qquad(\forall i\in[n']).
\end{align*}
We simultaneously claim that conditioned on events $E_1,...,E_n$ holding, and assuming $\sigma_*(x)\in\gamma(\sigma(x))$ for all $x\in\mathcal{X}$, then we have $\sigma_*'(x)\in\gamma(\sigma'(x))$ for all $x\in\mathcal{X}$. We prove by structural induction. The main requirement is that $\tilde{f}_{F,\delta}$ satisfies
\begin{align*}
\mathbb{P}(c\in\gamma(\tilde{f}_{F,\delta}(x_{\text{in}}))\mid E_1,...,E_n)\ge1-\delta.,
\end{align*}
where $F=[(E_1,\delta_1),...,(E_n,\delta_n)]$.

Skip: In this case, $n'=0$, so the first claim follows trivially. By induction, the second claim also follows trivially

Assign: In this case, $n'=0$, so the first claim follows trivially. By induction, we have $\sigma_*(x_i)\in\gamma(\sigma(x_i))$ for $i\in[k]$. By validity of $f^\#$, we have $f(\sigma_*(x_1),...,\sigma_*(x_k))\in\gamma(f^\#(\sigma(x_1),...,\sigma_k(x_k))$. After the update, we have $\sigma(x)=f^\#(\sigma(x_1),...,\sigma_k(x_k))$ and $\sigma_*(x)=f(\sigma_*(x_1),...,\sigma_*(x_k))$, so $\sigma_*(x)\in\gamma(\sigma(x))$, as claimed.

Assign': In this case, we have $n'=1$, and we need to show that $\mathbb{P}[E\mid E_1,...,E_n]\ge1-\delta$, where $E=\mathbbm{1}(c\in\gamma(a'))$ and $a'=\tilde{f}_{F,\delta}(x_{\text{in}})$. Indeed, this is the conformal guarantee provided by $\tilde{f}_{F,\delta}$, so the first claim follows. For the second claim, on event $E$, we have $c\in\gamma(a')$. Furthermore, by the same argument as above, we have $c\in\gamma(a)$. Thus, we have $c\in\gamma(a\sqcap a')$, so the claim follows.

Sequencing: We rewrite so that $F'$ becomes $F\circ F'$ and $F''$ becomes $F\circ F'\circ F''$. Then, by induction, for $p$, we have
\begin{align*}
\mathbb{P}[E_i'\mid E_1,...,E_k,E_1',...,E_{i-1}']\ge1-\delta_i'
\qquad(\forall i\in[k']),
\end{align*}
and for $p'$, we have
\begin{align*}
\mathbb{P}[E_i''\mid E_1,...,E_k,E_1',...,E_{k'}',E_1'',...,E_{i-1}'']\ge1-\delta_i''
\qquad(\forall i\in[k'']).
\end{align*}
Together, these two conditions are exactly the relationships required to show the first claim. For the second claim, by induction, the claim holds for $\sigma_*$



\clearpage
Let $\lambda=\mu^\#\otimes\mu_1\otimes...\otimes\mu_n$ be the product measure, and let $\tau=(\sigma^\#,\sigma_1,...,\sigma_n)$ be an element of the base space. We define a denotational semantics $\den{p}^\#_{\epsilon}:\mathcal{M}\mathcal{S}^\#\to\mathcal{M}\mathcal{S}^\#$.

Assign: $\den{\vec{x}\coloneqq f(\vec{x})}_{\epsilon}^\#(\lambda)=F_*(\lambda)$, where
\begin{align*}
F(\sigma^\#,\sigma_1,...,\sigma_n)=(f^\#(\sigma^\#),f(\sigma_1),...,f(\sigma_n))
\end{align*}

Assign-hat: $\den{\vec{x}\coloneqq\widehat{f}(\vec{x})}_{\epsilon}^\#(\lambda)=F_*(\lambda)$, where
\begin{align*}
F(\sigma^\#,\sigma_1,...,\sigma_n)=(C_{\epsilon}(\{f^*(\sigma_i)\}_{i=1}^n),f^*(\sigma_1),...,f^*(\sigma_n))
\end{align*}
We assume that for any $\mu$, we have
\begin{align*}
\mathbb{P}_{\mu(\sigma),\mu(\sigma_1),...,\mu(\sigma_n)}[f^*(\sigma)\in\gamma\circ C_{\epsilon}(\{f^*(\sigma_i)\}_{i=1}^n)]\ge1-\epsilon.
\end{align*}

Sequence: $\den{p;q}_{\epsilon}(\sigma^\#,\{\sigma_i\}_{i=1}^n=\den{p}_{\epsilon/2}(\den{q}_{\epsilon/2}(\sigma^\#,\{\sigma_i\}_{i=1}^n))$

Conditional:
\begin{align*}
\den{\textbf{if }x\textbf{ then }p\textbf{ else }q\textbf{ end}}_{\epsilon}^\#(\lambda)=\den{p}_{\epsilon}^\#\circ T_{B_1}(\lambda)+\den{q}_{\epsilon}^\#\circ T_{B_0}(\lambda)+F_*(\den{p}_{\epsilon}^\#\circ T_{B_{\top,1}}(\lambda)\otimes\den{q}_{\epsilon}^\#\circ T_{B_{\top,0}}(\lambda)),
\end{align*}
where
\begin{align*}
F((\sigma_1^\#,\sigma_{1,1}',...,\sigma_{1,n}'),(\sigma_0^\#,\sigma_{0,1}',...,\sigma_{0,n}'))
&=\delta(\sigma_1^\#\sqcup\sigma_0^\#,\sigma_1',...,\sigma_n')
~~\text{where}~~
\sigma_i'=\begin{cases}
\sigma_{1,i}'&\text{if }\sigma_i(x)=\text{true} \\
\sigma_{0,i}'&\text{if }\sigma_i(x)=\text{false},
\end{cases}
\end{align*}
and where
\begin{alignat*}{3}
&B_1&&=\{(\sigma^\#,\sigma_1',...,\sigma_n')\in\mathcal{T}\mid\sigma^\#(x)=\text{true}\}
\qquad&&\text{where}\qquad
\sigma_i'=\begin{cases}
\sigma_i&\text{if }\sigma_i(x)=\text{true} \\
\bot&\text{otherwise}
\end{cases} \\
&B_0&&=\{(\sigma^\#,\sigma_1',...,\sigma_n')\in\mathcal{T}\mid\sigma^\#(x)=\text{false}\}
\qquad&&\text{where}\qquad
\sigma_i'=\begin{cases}
\sigma_i&\text{if }\sigma_i(x)=\text{false} \\
\bot&\text{otherwise}
\end{cases} \\
&B_{\top,1}&&=\{(\sigma^\#,\sigma_1',...,\sigma_n')\in\mathcal{T}\mid\sigma^\#(x)=\top\}
\qquad&&\text{where}\qquad
\sigma_i'=\begin{cases}
\sigma_i&\text{if }\sigma_i(x)=\text{true} \\
\bot&\text{otherwise}
\end{cases} \\
&B_{\top,0}&&=\{(\sigma^\#,\sigma_1',...,\sigma_n')\in\mathcal{T}\mid\sigma^\#(x)=\top\}
\qquad&&\text{where}\qquad
\sigma_i'=\begin{cases}
\sigma_i&\text{if }\sigma_i(x)=\text{false} \\
\bot&\text{otherwise}
\end{cases} \\
\end{alignat*}

Consider the function
\begin{align*}
%\nu=\den{p}^*(\mu)\otimes\den{p}^\#_{\epsilon}(\alpha_*(\mu)\otimes\mu\otimes...\otimes\mu).
F(\sigma^*,\sigma^\#,\sigma_1,...,\sigma_n)=\delta(\sigma^*)\otimes\delta(\sigma^\#)\otimes\den{p}^*\circ\delta(\sigma^*)\otimes\den{p}^\#_{\epsilon}\circ\delta(\sigma^\#,\sigma_1,...,\sigma_n).
\end{align*}
Then, for any $\mu$ and $\mu^\#$, letting $\nu=F_*(\mu,\mu^\#,\mu,...,\mu)$, we claim that
\begin{align*}
\mathbb{P}_{\nu(\sigma^*,\sigma^\#,{\sigma^*}',({\sigma^\#}',\sigma_1',...,\sigma_n'))}[{\sigma^*}'\in\gamma({\sigma^\#}')\mid\sigma^*\in\gamma(\sigma^\#)]\ge1-\epsilon.
\end{align*}

Proof:
\begin{itemize}
\item Assuming the input distributions are all equal (i.e., $\lambda=\mu\otimes\mu^\#\otimes\mu\otimes...\otimes\mu$), then the semantics are same for $\sigma,\sigma_1,...,\sigma_n$ (i.e., $\pi_i(\den{p}_{\epsilon}^C(\lambda)=\pi_j(\den{p}_{\epsilon}^C(\lambda)$, where $\pi_i$ is the projection onto component $i$), and equal the ground truth semantics (i.e., $\pi_i(\den{p}_{\epsilon}^C(\lambda)=\den{p}^*(\lambda)$). Proof: In general, we have $\pi_i(\den{p}_{\epsilon}^C(\lambda))=\den{p}^*(\mu_i)$. This holds by structural induction; for while loops, this holds by taking the projection of the equation and noting that it is equivalent to the equation for the ground truth semantics. Then, everything else follows.
\item Assuming the input distributions are all equal, then 
\end{itemize}



Now, we prove Theorem~\ref{thm:impmain}
\begin{proof}
We prove by structural induction on $p$. First, consider an assignment with a standard component $f\in\mathcal{F}$. Conditioned on the event $\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)$, we have
\begin{align*}
\den{p}^*(\sigma_*)=f(\sigma_*)\in\gamma(f^\#(\sigma_\#))=\gamma(\den{p}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n)),
\end{align*}
so the desired event holds with probability one, and the claim follows. Next, consider an assignment with a machine learning component $\widehat{f}\in\widehat{\mathcal{F}}$. We have
\begin{align*}
&\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\sigma_*\in C_{\epsilon}(\{f^*(\sigma_i)\}_{i=1}^n)\mid\sigma_*\neq\bot] \\
&=\mathbb{P}_{\pi_*(\lambda)(\{\sigma_i\}_{i=1}^n,\sigma_*)}[\sigma_*\in C_{\epsilon}(\{f^*(\sigma_i)\}_{i=1}^n)\mid\sigma_*\neq\bot] \\
&=\mathbb{P}_{\mu(\sigma_1),...,\mu(\sigma_n),\mu(\sigma_*)}[\sigma_*\in C_{\epsilon}(\{f^*(\sigma_i)\}_{i=1}^n)\mid\sigma_*\neq\bot] \\
&\ge1-\epsilon,
\end{align*}
where the first equality follows since the event and condition do not depend on $\sigma_\#$ (and by change of measure), the second equality follows by our assumption on $\lambda$, and the inequality follows by our conformal guarantee in Lemma~\ref{lem:impconformal}. Next, consider a sequence $p;q$. By induction, we have
\begin{align}
\label{eqn:impproof:seq:1}
\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{p}^*(\sigma_*)\in\gamma(\den{p}^C_{\epsilon/2}(\sigma_\#,\{\sigma_i\}_{i=1}^n))\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)]\ge1-\frac{\epsilon}{2}.
\end{align}
In addition, let $E=\{(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)\mid\sigma_*\in\gamma(\sigma_\#)\}$ be the event that $\sigma_*\in\gamma(\sigma_\#)$, and define the define the conditional probability measure $\tilde{\lambda}(A)=\lambda(E\cap A)/\lambda(E)$, which is well defined since $\lambda(E)>0$ by assumption. It is easy to check that $\tilde{\lambda}$ satisfies $\pi_*(\tilde{\lambda})=\otimes_{i=1}^n\den{p}^*_*(\mu)$. Now, let $\nu=\den{p}^J_{\epsilon/2,*}(\tilde{\lambda})$. Then, by Lemma~\ref{lem:TODO}, we have $\pi_*(\nu)=\otimes_{i=1}^n\den{p}^*_*(\mu)$, so it satisfies the assumption of our induction hypothesis. Thus, by induction, we have
\begin{align}
\label{eqn:impproof:seq:2}
\mathbb{P}_{\nu(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*)\in\gamma(\den{q}^C_{\epsilon/2}(\sigma_\#,\{\sigma_i\}_{i=1}^n))\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)]\ge1-\frac{\epsilon}{2}.
\end{align}
Now, consider the complement of the probability we need to bound:
\begin{align*}
&\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*')\not\in\gamma(\den{q}^C_{\epsilon/2}(\sigma_\#',\{\sigma_i'\}_{i=1}^n))\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*')\in\gamma(\den{q}^C_{\epsilon/2}(\sigma_\#',\{\sigma_i'\}_{i=1}^n))\wedge\sigma_*'\in\gamma(\sigma_\#')\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&\qquad+\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*')\in\gamma(\den{q}^C_{\epsilon/2}(\sigma_\#',\{\sigma_i'\}_{i=1}^n))\wedge\sigma_*'\not\in\gamma(\sigma_\#')\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&\le\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*')\in\gamma(\den{q}^C_{\epsilon/2}(\sigma_\#',\{\sigma_i'\}_{i=1}^n))\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)\wedge\sigma_*'\in\gamma(\sigma_\#')] \\
&\qquad+\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\sigma_*'\not\in\gamma(\sigma_\#')\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&\le\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*')\in\gamma(\den{q}^C_{\epsilon/2}(\sigma_\#',\{\sigma_i'\}_{i=1}^n))\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)\wedge\sigma_*'\in\gamma(\sigma_\#')]+\frac{\epsilon}{2} \\
&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*')\in\gamma(\den{q}^C_{\epsilon/2}(\sigma_\#',\{\sigma_i'\}_{i=1}^n))\mid\sigma_*'\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)\wedge\sigma_*'\in\gamma(\sigma_\#')]+\frac{\epsilon}{2} \\
&=\mathbb{P}_{\nu(\sigma_\#',\{\sigma_i'\}_{i=1}^n,\sigma_*')}[\den{q}^*(\sigma_*')\in\gamma(\den{q}^C_{\epsilon/2}(\sigma_\#',\{\sigma_i'\}_{i=1}^n))\mid\sigma_*'\neq\bot\wedge\sigma_*'\in\gamma(\sigma_\#')]+\frac{\epsilon}{2} \\
&\le\epsilon,
\end{align*}
where the first equality follows by the law of total probability, the first inequality follows since the conditional probability is greater than or equal to the probability of the event (for the first term), and the probability of an event is less than or equal to the probability of either event (for the second term), the second inequality follows since the second term is $<\epsilon/2$ by (\ref{eqn:impproof:seq:1}), the second equality follows since $\sigma_*=\bot$ is equivalent to $\sigma_*'=\bot$ by Lemma~\ref{lem:TODO}, the third equality follows by change of measure, and the last inequality follows since the first term is $<\epsilon/2$ by (\ref{eqn:impproof:seq:2}).  The claim follows.

For conditionals, letting $q=\textbf{if }x\textbf{ then }p$, consider the probability of the complement of the event we want to bound:
\begin{align*}
&\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*)\not\in\gamma(\den{q}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n))\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*)\not\in\gamma(\den{q}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n))\wedge\sigma_*(x)=\text{true}\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&\qquad+\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*)\not\in\gamma(\den{q}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n))\wedge\sigma_*(x)=\text{false}\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*)\not\in\gamma(\den{q}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n))\wedge\sigma_*(x)=\text{true}\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)],
\end{align*}
where the last line follows because for the second term, if $\sigma_*(x)=\text{false}$, then $\den{q}^*(\sigma_*)=\sigma_*$; furthermore, on the event $\sigma_*\in\gamma(\sigma_\#)$, we have $\text{false}\in\gamma(\sigma_\#)$, so it follows that $\den{q}^*(\sigma_*)\in\gamma(\den{q}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n))$ with probability one. For the remaining term, note that since $\sigma_*(x)=\text{true}$, we have $\den{q}^*(\sigma_*)=\den{p}^*(\sigma_*)$; furthermore, on the event $\sigma_*\in\gamma(\sigma_\#)$, we have $\text{true}\in\gamma(\sigma_\#)$, so it follows that
\begin{align*}
\gamma(\den{p}^C_{\epsilon}(\iota_{\text{true}}(\sigma_\#),\{\iota_{\text{true}}(\sigma_i)\}_{i=1}^n))\subseteq\gamma(\den{q}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n)).
\end{align*}
As a consequence, we have
\begin{align*}
&\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{q}^*(\sigma_*)\not\in\gamma(\den{q}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n))\wedge\sigma_*(x)=\text{true}\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{p}^*(\iota_{\text{true}}(\sigma_*))\not\in\gamma(\den{q}^C_{\epsilon}(\sigma_\#,\{\sigma_i\}_{i=1}^n))\wedge\sigma_*(x)=\text{true}\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&\le\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{p}^*(\iota_{\text{true}}(\sigma_*))\not\in\gamma(\den{p}^C_{\epsilon}(\iota_{\text{true}}^\#(\sigma_\#),\{\iota_{\text{true}}(\sigma_i)\}_{i=1}^n))\wedge\sigma_*(x)=\text{true} \\
&\hspace{4in}\mid\sigma_*\neq\bot\wedge\sigma_*\in\gamma(\sigma_\#)] \\
&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{p}^*(\iota_{\text{true}}(\sigma_*))\not\in\gamma(\den{p}^C_{\epsilon}(\iota_{\text{true}}^\#(\sigma_\#),\{\iota_{\text{true}}(\sigma_i)\}_{i=1}^n))\wedge\sigma_*(x)=\text{true} \\
&\hspace{3in}\mid\iota_{\text{true}}(\sigma_*)\neq\bot\wedge\iota_{\text{true}}(\sigma_*)\in\gamma(\iota_{\text{true}}^\#(\sigma_\#))] \\
&\le\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{p}^*(\iota_{\text{true}}(\sigma_*))\not\in\gamma(\den{p}^C_{\epsilon}(\iota_{\text{true}}^\#(\sigma_\#),\{\iota_{\text{true}}(\sigma_i)\}_{i=1}^n)) \\
&\hspace{3in}\mid\iota_{\text{true}}(\sigma_*)\neq\bot\wedge\iota_{\text{true}}(\sigma_*)\in\gamma(\iota_{\text{true}}^\#(\sigma_\#))] \\
&=\mathbb{P}_{G_*(\lambda)(\sigma_\#',\{\sigma_i'\}_{i=1}^n,\sigma_*')}[\den{p}^*(\sigma_*')\not\in\gamma(\den{p}^C_{\epsilon}(\sigma_\#',\{\sigma_i'\}_{i=1}^n))\mid\sigma_*'\neq\bot\wedge\sigma_*'\in\gamma(\sigma_\#')] 
\end{align*}
By Lemma~\ref{lem:TODO} with $g^\#=\iota_{\text{true}}^\#$ and $g=\iota_{\text{true}}$, we have $\pi_*\circ G_*(\lambda)=\otimes_{i=1}^{n+1}g_*(\mu)$. Thus, by structural induction, we have
\begin{align*}
\mathbb{P}_{G_*(\lambda)(\sigma_\#',\{\sigma_i'\}_{i=1}^n,\sigma_*')}[\den{p}^*(\sigma_*')\in\den{p}^C_{\epsilon}(\sigma_\#',\{\sigma_i'\}_{i=1}^n)\mid\sigma_*'\neq\bot\wedge\sigma_*'\in\gamma(\sigma_\#')]\ge1-\epsilon.
\end{align*}
Now, considering the probability of the complement of the event, we have
\begin{align*}
&\mathbb{P}_{G_*(\lambda)(\sigma_\#',\{\sigma_i'\}_{i=1}^n,\sigma_*')}[\den{p}^*(\sigma_*')\not\in\den{p}^C_{\epsilon}(\sigma_\#',\{\sigma_i'\}_{i=1}^n)\mid\sigma_*'\neq\bot\wedge\sigma_*'\in\gamma(\sigma_\#')] \\
&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{p}^*(\sigma_*')\not\in\den{p}^C_{\epsilon}(\sigma_\#',\{\sigma_i'\}_{i=1}^n)\mid\sigma_*'\neq\bot\wedge\sigma_*'\in\gamma(\sigma_\#')] \\
&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{p}^*(\sigma_*')\not\in\den{p}^C_{\epsilon}(\sigma_\#',\{\sigma_i'\}_{i=1}^n)\mid\sigma_*\neq\bot\wedge\sigma_*'\in\gamma(\sigma_\#')\wedge\sigma_*(x)=\text{true}] \\
%&=\mathbb{P}_{\lambda(\sigma_\#,\{\sigma_i\}_{i=1}^n,\sigma_*)}[\den{p}^*(\sigma_*')\not\in\den{p}^C_{\epsilon}(\sigma_\#',\{\sigma_i'\}_{i=1}^n)\mid\sigma_*\neq\bot\wedge\sigma_*'\in\gamma(\sigma_\#')\wedge\sigma_*(x)=\text{true}] \\
\end{align*}
the first equality follows by change of measure, the second because $\sigma_*'=\iota_{\text{true}}(\sigma_*)\neq\bot$ iff $\sigma=\bot$ or $\sigma(x)=\text{true}$.


Now, considering the probability of the complement of the event, we have
\begin{align*}
&\mathbb{P}_{G_*(\lambda)(\sigma_\#',\{\sigma_i'\}_{i=1}^n,\sigma_*')}[\den{p}^*(\sigma_*')\not\in\den{p}^C_{\epsilon}(\sigma_\#',\{\sigma_i'\}_{i=1}^n)\mid\sigma_*'\neq\bot\wedge\sigma_*'\in\gamma(\sigma_\#')] \\
\end{align*}
\end{proof}


==> programs.tex <==

\textbf{Programs} \ramya{Should add these as column to table}\textbf{:}\\
Program 1 (Total number of people + cars in image): \\
$p_1~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person}\vee d_1=\textsf{car})))~(\widehat{f}~X)~0)$\\
Program 2 (Number of people within 100 pixels of left side of image): \\
$p_2~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person}\wedge d_2\le100)))~(\widehat{f}~X)~0)$ \\
Program 3 (Number of people within 100 pixels of bottom of image): \\
$p_3~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person}\wedge d_3\le100)~(\widehat{f}~X)))~0)$ \\
Program 4 (Number of people within 100 pixels of top of image): \\
$p_4~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person}\wedge d_3\ge\textsf{MAX-HEIGHT} - 100)~(\widehat{f}~X)))~0)$ \\
Program 5 (Number of people within 100 pixels of right side of image): \\
$p_5~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person}\wedge d_2\ge\textsf{MAX-WIDTH} - 100)~(\widehat{f}~X)))~0)$ \\
Program 6 (Number of cars within 100 pixel distance of a person): \\
$p_6~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,(d_{1,2} - d_{2,2})^2 + (d_{1,3} - d_{2,3})^2 \leq 100^2)~((\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person})~(\widehat{f}~X)) \times (\textsf{filter}~(\lambda d\,.\,d_1=\textsf{car})~(\widehat{f}~X)))))~0)$ \\
Program 7 (Number of people within 100 pixels to the left of a car):\\
$p_7~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_{1, 2} \leq d_{2, 2} \wedge (d_{1,2} - d_{2,2})^2 + (d_{1,3} - d_{2,3})^2 \leq 100^2)~((\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person})~(\widehat{f}~X)) \times (\textsf{filter}~(\lambda d\,.\,d_1=\textsf{car})~(\widehat{f}~X)))))~0)$ \\
Program 8 (Number of people within 100 pixels to the right of a car): \\
$p_8~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_{1, 2} \geq d_{2, 2} \wedge (d_{1,2} - d_{2,2})^2 + (d_{1,3} - d_{2,3})^2 \leq 100^2)~((\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person})~(\widehat{f}~X)) \times (\textsf{filter}~(\lambda d\,.\,d_1=\textsf{car})~(\widehat{f}~X)))))~0)$ \\
Program 9 (Number of people within 100 pixels below a car): \\
$p_9~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_{1, 3} \leq d_{2, 3} \wedge (d_{1,2} - d_{2,2})^2 + (d_{1,3} - d_{2,3})^2 \leq 100^2)~((\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person})~(\widehat{f}~X)) \times (\textsf{filter}~(\lambda d\,.\,d_1=\textsf{car})~(\widehat{f}~X)))))~0)$ \\
Program 10 (Number of people within 100 pixels above a car): \\
$p_{10}~=~(\textsf{foldr}~+~(\textsf{map}~(\lambda d\,.\,1)~(\textsf{filter}~(\lambda d\,.\,d_{1, 3} \geq d_{2, 3} \wedge (d_{1,2} - d_{2,2})^2 + (d_{1,3} - d_{2,3})^2 \leq 100^2)~((\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person})~(\widehat{f}~X)) \times (\textsf{filter}~(\lambda d\,.\,d_1=\textsf{car})~(\widehat{f}~X)))))~0)$ \\
Program 11 (Minimum distance between two people): \\
$p_{11}~=~(\textsf{foldr}~\textsf{min}~(\textsf{map}~(\lambda d\,.\,\sqrt{(d_{1,2} - d_{2, 2})^2 + (d_{1,3} - d_{2,3})^2})~((\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person})~(\widehat{f}~X)) \times (\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person})~(\widehat{f}~X))))~\infty)$ \\
Program 12 (Maximum distance between a car and a person): \\
$p_{12}~=~(\textsf{foldr}~\textsf{max}~(\textsf{map}~(\lambda d\,.\,\sqrt{(d_{1,2} - d_{2, 2})^2 + (d_{1,3} - d_{2,3})^2})~((\textsf{filter}~(\lambda d\,.\,d_1=\textsf{car})~(\widehat{f}~X)) \times (\textsf{filter}~(\lambda d\,.\,d_1=\textsf{person})~(\widehat{f}~X))))~0)$ \\
\\

